Cu\'anto es demasiada inflaci\'on? Una clasificaci\'on de reg\'imenes inflacionarios

The classifications of inflationary regimes proposed in the literature have mostly been based on arbitrary characterizations, subject to value judgments by researchers. The objective of this study is to propose a new methodological approach that reduces subjectivity and improves accuracy in the construction of such regimes. The method is built upon a combination of clustering techniques and classification trees, which allows for an historical periodization of Argentina's inflationary history for the period 1943-2022. Additionally, two procedures are introduced to smooth out the classification over time: a measure of temporal contiguity of observations and a rolling method based on the simple majority rule. The obtained regimes are compared against the existing literature on the inflation-relative price variability relationship, revealing a better performance of the proposed regimes.

==> Basurero_de_texto.tex <==
Sobre HyL
%Este criterio resulta inadecuado, ya que considera en un mismo régimen a economías con dinámicas inflacionarias que potencialmente pueden ser muy distintas.

Debido a que el algoritmo de $k$-medias no puede emplearse con una matriz de distancias, es necesario transformar la matriz de DCT de dimensión ($T \times T$) en una matriz de la forma ($p \times T$). Para lograr esto, se emplea el análisis de coordenadas principales, el cual proporciona una representación euclídea de la matriz DCT en el espacio de las $p$ variables, obteniendo como resultado una matriz ($p \times T$). Posteriormente, se aplica el método de $k$-medias a esta matriz transformada.

% De esta forma, se consideran regímenes inflacionarios como ``hiperinflación'', ``inflación alta'' e ``inflación moderada'', que se caracterizan por un cierto rango numérico provisto para la tasa de inflación.


%A diferencia de las definiciones previas donde la unidad temporal presenta un rol secundario, para \textcite{harberger1978} le presencia de la denominada ``inflación crónica'' en tasas de más de un 20\% anual por largos períodos de tiempo pasa a ser el centro de atención, la cual pone en contraste con la ``inflación aguda'' caracterizada por subas abruptas de precios en tasas por encima del 80\% anual por al menos tres años.

%Por último, queda pendiente el estudio de la dinámica de diferentes relaciones económicas en los regímenes propuestos, como inflación-variación de precios relativos, para luego comparar los resultados con la literatura existente en la materia.

\begin{table}
\begin{center}
\begin{tabular}{l c}
\hline
 & Model 1 \\
\hline
mu             & $0.019^{***}$ \\
               & $(0.007)$     \\
omega          & $0.000^{**}$ \\
               & $(0.000)$     \\
alpha1         & $0.206^{***}$ \\
               & $(0.015)$     \\
beta1          & $0.793^{***}$ \\
               & $(0.012)$     \\
\hline
Num. obs.      & $959$        \\
AIC            & $-4.66$      \\
Log Likelihood & $2240.452$   \\
\hline
\multicolumn{2}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}

\label{table:coefficients}
\end{center}
\end{table}

La inflación, al deteriorar el poder de compra de los consumidores y generar incertidumbre en los mercados, acarrea costos sustanciales para las economías. Por ende, comprender y analizar las dinámicas de los procesos inflacionarios resulta fundamental para la adecuada formulación de políticas públicas.

Las economías poseen dinámicas muy diversas de acuerdo con la tasa de inflación que experimentan. Es por ello que la literatura empírica ha creado categorías conocidas como ``regímenes inflacionarios'' para estudiar estos procesos.

Sin embargo, el estudio de la inflación presenta desafíos debido a su naturaleza multifacética y a menudo impredecible. 

Algo sobre las distintas dinamicas y entender mejor el proceso inflacionario
La inflación es un fenómeno económico persistente y a menudo desafiante que ha sido ampliamente estudiado por los economistas

A pesar de ser la inflación uno de los temas más estudiados por la ciencia económica en el siglo XX, diversos aspectos en torno a su caracterización han sido vagamente estudiados por la literatura. Es así que la noción de ``régimen inflacionario'' suele ser utilizada de forma implícita a lo largo de muchos estudios, los cuales caracterizan un cierto período temporal como de ``alta inflación'' o de ``hiperinflación'', pero sin dejar clara su definición, ni mucho menos sus umbrales.

Generalizan, intentando crear una vision universal de fenomenos heterogeneos. No contemplan que cada pais puede tener un proceso inflacionario de caracteristicas diversas dada por la endogeneidad del proceso






% TODO LO DE GARCH Y VOLATILIDAD:

Se consideró como variables de agrupamiento para el análisis de \textit{clusters} a la tasa de inflación mensual y a su volatilidad.
Los datos de la tasa de inflación mensual provienen del INDEC, mientras que la volatilidad de la inflación es estimada


Existen diversas alternativas en la literatura para generar una medida de la variabilidad de la inflación. Entre estas, se destacan el valor absoluto de la primera diferencia de la serie \parencite{khan1977}, el desvío estándar de la tasa de inflación para un cierto período \parencite{taylor1981} y la desviación absoluta de la tasa de inflación con respecto a una media móvil de la misma \parencite{dabus1994}. La elección de estas medidas de volatilidad ha sido cuestionada por autores como \textcite{engle1982uk} debido a la arbitrariedad que implican y la falta de coherencia con el enfoque econométrico tradicional. Por este motivo, se decidió adoptar el método estándar en la literatura y estimar la volatilidad utilizando modelos de tipo ARCH, siendo la volatilidad representada por la varianza condicional estimada de la tasa de inflación mensual (\cite{engle1982uk,engle1983usa}). Para ello, primero se evaluó la presencia de efectos ARCH y posteriormente se estimó la variabilidad mediante un modelo GARCH (1,1), debido a su parsimonia y excelente capacidad predictiva \parencite{hansen2005}. Los detalles de la estimación son presentados en el Apéndice \ref{appendix:appA}.

\subsection{Estimaciones con volatilidad}

% De aca voy a concluir del CART que la volatilidad no es relevante para predecir el regimen inflacionario y, que por ende, me quedo solo con la tasa de inflación.


Debido a la baja relevancia de la volatilidad en la construcción de los regímenes, se procede a analizar las estimaciones de realizadas únicamente con la tasa de inflación como variable de clasificación.

%
\appendix

\section{Estimación de la volatilidad} 
\label{appendix:appA}
Antes de proceder con la estimación, se debe verificar la presencia de efectos ARCH. Para ello, primero se estima un modelo ARIMA (5,1,4) elegido en base al criterio de información de Akaike (AIC) por la función \textit{auto.arima} del paquete \textit{forecast} en R \parencite{autoarima}. Posteriormente, se evaluó la presencia de efectos autorregresivos en la varianza del modelo estimado mediante la prueba Q de Portmanteau y la prueba del multiplicador de Lagrange de \textcite{engle1982uk}. Los resultados de los tests se detallan en la Tabla \ref{tab:tabARCH}. De la misma se concluye en favor de la presencia de efectos ARCH en el modelo ARIMA estimado.

\input{test_arch}

En base a los resultados previos, se procede a estimar un modelo GARCH (1,1), del cual se extrae el componente de varianza condicionada para utilizar como \textit{proxy} de la volatilidad de la inflación. La siguiente tabla presenta los resultados del modelo estimado.

\input{tabGARCH}



%\begin{tabular}{lccc}
%\multicolumn{4}{@{}l}{\small Pruebas de diferencia de medias}\\
%\multicolumn{4}{c}{}\\[-1em]
%\hline
%Regí­menes & Inflación promedio & Fisher & Tukey \\ 
%\hline
%Inflación baja & 1,36 & a & a \\ 
%Inflación moderada & 8,66 & b & b \\ 
%Inflación alta & 24,30 & c & c \\
%Hiperinflación & 112,86 & d & d \\
%\hline
%\end{tabular}


==> regs_dabus.tex <==
\begin{table}[H]
\begin{center}
\caption{Regresiones inflación-precios relativos \label{tab:comp_dab_reg}}
\vspace{2mm}
\footnotesize
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{5}{c}}
\hline
            & (1) & (2) & (3) & (4) & (5)\\
            & VPR & VPR & VPR & VPR & VPR\\
\hline
\multicolumn{6}{c}{}\\[-0.9em]
 & \textbf{Base} & \textbf{$k$-medias} & \textbf{DCT} & \textbf{MS} & \textbf{Dabús}\\
[0.4em]
INF        &      0.0069\sym{***}&      0.0076         &      0.0076         &      0.0140         &      0.0075         \\
            &    (0.0007)         &    (0.0110)         &    (0.0124)         &    (0.0094)         &    (0.0206)         \\
[0.5em]
MOD     &                     &      0.0007         &     -0.0011         &      0.0010\sym{*}  &     -0.0001         \\
            &                     &    (0.0011)         &    (0.0008)         &    (0.0005)         &    (0.0007)         \\
[0.5em]
ALTA     &                     &      0.0006         &     -0.0036\sym{**} &      0.0045         &     -0.0007         \\
            &                     &    (0.0024)         &    (0.0013)         &    (0.0059)         &    (0.0009)         \\
[0.5em]
HIPER     &                     &      0.0033         &      0.0033         &      0.0097\sym{***}&      0.0094\sym{***}\\
            &                     &    (0.0020)         &    (0.0020)         &    (0.0011)         &    (0.0016)         \\
[0.5em]
MOD $*$ INF &                     &      0.0051         &      0.0294         &     -0.0062         &      0.0044         \\
            &                     &    (0.0152)         &    (0.0155)         &    (0.0096)         &    (0.0255)         \\
[0.5em]
ALTA $*$ INF &                     &      0.0158         &      0.0245         &      0.0000         &      0.0213         \\
            &                     &    (0.0123)         &    (0.0128)         &         (.)         &    (0.0210)         \\
[0.5em]
HIPER $*$ INF &                     &     -0.0055         &     -0.0055         &     -0.0154         &     -0.0091         \\
            &                     &    (0.0111)         &    (0.0125)         &    (0.0095)         &    (0.0206)         \\
[0.5em]
Constante      &      0.0003\sym{*}  &      0.0001         &      0.0001         &      0.0000         &      0.0001         \\
            &    (0.0001)         &    (0.0001)         &    (0.0001)         &    (0.0001)         &    (0.0001)         \\
\multicolumn{6}{c}{}\\[-1.1em]
\hline
\multicolumn{6}{c}{}\\[-1.1em]
\(R^{2}\) ajustado &       0.297         &       0.595         &       0.608         &       0.561         &       0.558         \\
\textit{AIC}&     -2057.1         &     -2167.0         &     -2173.8         &     -2150.8         &     -2148.6         \\
\textit{BIC}&     -2050.4         &     -2140.2         &     -2147.0         &     -2127.3         &     -2121.9          \\
\textit{RMSE}        &      0.0018         &      0.0014         &      0.0013         &      0.0014         &      0.0014         \\
Observaciones       &         210         &         210         &         210         &         210         &         210         \\
\multicolumn{6}{c}{}\\[-1.1em]
\hline
\multicolumn{6}{c}{}\\[-1.1em]
\textit{F} (Chow)       &      -         &      26.50         &      28.47         &      25.92         &      21.46         \\
p-valor      &         -         &         0.000         &         0.000         &         0.000         &         0.000         \\
\multicolumn{6}{c}{}\\[-1.1em]
\hline
\multicolumn{6}{c}{}\\[-1.1em]
\multicolumn{6}{l}{\footnotesize Nota: Desvíos estándar entre paréntesis.
}\\
\multicolumn{6}{l}{\footnotesize *, **, *** indican significatividad al 5\%, 1\% y 0,1\% , respectivamente.
}\\
\end{tabular}
}
\end{center}
\vspace{-0.5cm}
\end{table}
%\sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)

==> tabGARCH.tex <==
\begin{table}[H]
\begin{center}
\caption{Estimación modelo GARCH (1,1) \label{tab:tabGARCH}}
\vspace{2mm}
\small
\begin{tabular}{lcccc}
\hline
Parámetro &  Coeficiente & Error estándar &  Estadístico t & p-valor \\ 
\hline
\multicolumn{2}{l}{Ecuación de la media condicional} & & & \\
$\mu$ & 0.019 & 0.007 & 2.626 & 0.009 \\ 
AR (1) & 0.974 & 0.011 & 89.845 & 0.000 \\ 
MA (1) & -0.548 & 0.048 & -11.405 & 0.000 \\
\multicolumn{2}{l}{Ecuación de la varianza condicional} & & & \\
$\omega$ & 0.000 & 0.000 & 2.261 & 0.024 \\ 
$\alpha_1$ & 0.206 & 0.015 & 14.026 & 0.000 \\ 
$\beta_1$ & 0.793 & 0.012 & 66.432 & 0.000 \\ 
 \hline
\end{tabular}
\end{center}
\end{table}


==> test_arch.tex <==
\begin{table}[h]
\begin{center}
\caption{Pruebas de efectos ARCH}
\label{tab:tabARCH}
\vspace{2mm}
\small
\begin{tabular}{ccccc}
\hline
Rezagos & PQ & p-value & LM & p-value \\ 
\hline
4 & 430.04 & 0.000 & 311.24 & 0.000 \\ 
8 & 432.26 & 0.000 & 144.06 & 0.000 \\ 
12 & 442.65 & 0.000 & 93.11 & 0.000 \\ 
16 & 444.51 & 0.000 & 68.84 & 0.000 \\ 
24 & 444.66 & 0.000 & 44.83 & 0.004 \\ 
\hline
\end{tabular}
\end{center}
\vspace{-0.5cm}
\end{table}
